Real-Time Quadrotor Trajectory Optimization with Time-Triggered Corridor Constraints

One of the keys to flying quadrotors is to optimize their trajectories within the set of collision-free corridors. These corridors impose nonconvex constraints on the trajectories, making real-time trajectory optimization challenging. We introduce a novel numerical method that approximates the nonconvex corridor constraints with time-triggered convex corridor constraints. This method combines bisection search and repeated infeasibility detection. We further develop a customized C++ implementation of the proposed method, based on a first-order conic optimization method that detects infeasibility and exploits problem structure. We demonstrate the efficiency and effectiveness of the proposed method using numerical simulation on randomly generated problem instances as well as indoor flight experiments with hoop obstacles. Compared with mixed integer programming, the proposed method is about 50--200 times faster.

==> experiment/experiment.tex <==
\subsection{Flight experiments with hoop obstacles}

The multi-rotors we consider are capable of generating only one force and three torques, and thus cannot simultaneously control the six degrees-of-freedom along which they evolve.

\input{experiment/figs/quad}

\subsubsection{Hardware}

The hardware of the quadrotor includes a set of actuators, sensors, and processors.

\paragraph{Actuators}
Our quadrotor has four actuators, each consists of a variable-speed brushless direct current motor and a fixed-pitch variable-revolutions-per-minute propeller. Each motor is powered by a 2200-milliAmp-hour lithium-polymer battery that provides a flight time of 15-30 minutes. Each propeller generates a thrust, produced by the lifting force of the propeller blades, and a torque, produced by the drag force of the propeller blades.

\paragraph{Sensors}
Our quadrotor has access to the following two set of sensors.
\begin{enumerate}
    \item On-board sensors: The quadrotor has two set of on-board sensors: accelerometers and gyroscopes, which measure the acceleration and the angular velocity, respectively, at a 100-1000 Hertz (Hz) rate.
    \item Off-board sensors: The quadrotor also has access to an OptiTrack motion capture system that measures attitude and position at 50-150 Hz rate.
\end{enumerate}

\paragraph{Processors}
The on-board electronics include a inertial measurement unit, a 500 MHz dual-core Intel Edison, a 1.7 GHz quad-core Intel Joule, and an IEEE 802.11n compliant WiFi communication link.

\subsubsection{Software}

\input{experiment/figs/diagram}

We developed a feedback-control software architecture, illustrated in Fig.~\ref{fig: diagram}, to track the trajectory computed by Algorithm~\ref{alg: trigger}. Such architecture contains four different blocks: controller, allocator \& converter, actuator, ans sensor. We will explain the function and ideas of each block in the following. 

\paragraph{Controller}
The controller block takes the input trajectory computed by Algorithm~\ref{alg: trigger}, which is in the inertial frame of reference, as input, and outputs a \emph{wrench trajectory} in the body frame of reference. This trajectory is composed of a collection of wrench vector; each wrench vector includes three torques and one force. The controller contains three separate layers of proportional-integral-derivative controllers. These layers address several technical challenges including the time-varying mismatch between the inertial frame and body frame of reference, the bias and time-delays of the sensor measurements, actuator saturation, and external force and torque disturbances. The design of these controllers is based on the nonlinear dynamic compensator and loop-shaping techniques \cite[Chp. 6]{szmuk2019successive}.

\paragraph{Allocator \& converter}
The allocator and converter block takes the output of the controller block as inputs, and outputs the command signals for the onboard motors of the quadrotor. In particular, the allocator computes a physically realizable wrench command that most closely matches the output of the controller. Such computation is based on solving a sequence of linear programs in a lexicographic ordering that ensures a collection of prioritization properties \cite[Sec. 6.4]{szmuk2019successive}. The converter converts each wrnch vector computed by the allocator to pulse-width-modualted signals that are subsequently sent to the on-board motors. The conversion is based on a quadratic formula between motor force and brushless DC electric motor commands \cite[Sec. 6.3]{szmuk2019successive}.  

\subsection{Flight experiments}



==> experiment/feedback.tex <==


\section{Skye: Quadrotor Feedback Control Draft}
\label{sec: feedback2}

Citation: Chapter 6 of Miki's dissertation.

To achieve high-performance agile flight experiments with our quadrotor drones, we combine both feed-forward guidance and feedback control. The feed-forward guidance is produced via our real-time trajectory generation algorithms, which are both forward-looking and allow us to consider both optimality and constraints when planning the vehicle's motion. However, feed-forward methods have limitations as they are sensitive to model uncertainties and external disturbances. To counteract this, the control terms generated by our trajectory generation algorithms are ignored. Instead, the generated optimal time history of quadrotor states including Cartesian and angular position, velocity, and acceleration are passed as a reference trajectory into a high-order on-board feedback controller. Feedback control is robust to model uncertainties and external disturbances, but is in nature myopic and does not consider state constraints. In this way, we combine the optimality and constraint satisfaction benefits of feed-forward guidance with the robustness and performance guarantees of feedback control to execute aggressive trajectory tracking on-board the quadrotor drones in real-time.

The use of a high-order feedback controller on-board the quadrotor flight computer also enables the use of a convex simplified dynamic model to constrain the optimal control problem. This simplified model assumes 3 degree of freedom (DoF) translational motion of the drone. However, in reality the 6-DoF dynamics of the vehicle have a coupling between the translational and attitude state evolution. The feedback controllers on-board account for this discrepancy, and this coupling will become important later in the allocation step of the underlying controller.

First, the high-level controller is commanded by a trajectory specified through five inputs: inertial position, a specified force, a reference attitude, an angular velocity, and a torque. This high-level controller also receives feedback on the inertial position and attitude via the motion-capture system, as well as acceleration measured by an accelerometer on-board. This controller then passes a series of four outputs as inputs to the mid-level controller: a commanded force along the negative vehicle Z-axis, a commanded body-frame attitude and attitude rate, and a commanded body-frame torque. In principle, these inputs can be in any arbitrary frame denoted as the "mid-level frame", but in practice this frame is the body-frame. This mid-level controller also receives feedback on the vehicle attitude via the motion-capture systems, as well as the body-rates from an on-board gyroscope. Finally, this mid-level controller computes four commands that are passed as inputs to the low-level controller in the body-frame: a force of thrust along the vehicle's negative Z-axis, a feed-forward torque, a feed-forward body rate, and a feedback body rate. This low-level controller also receives feedback on the body rates and acceleration from on-board sensors. This low-level controller then produces a single vector output: a requested wrench, which consists of a force and three torques about the vehicle body-frame axes. 

Due to the aforementioned coupling between the vehicle's translational and attitude dynamics, the requested wrench cannot necessarily be achieved instantaneously; the vehicle must adjust it's attitude in the inertial frame in order to vary how the body frame torques and forces are evolving the vehicle's motion in the inertial frame. Due to this, an arbitrary set of attitudes and positions (and their rates) cannot be achieved instantaneously at any point along the trajectory. To account for this, an allocator produces a series of projections that prioritize the requested torques and force, before producing a dynamically feasible wrench that is the closest possible to the requested wrench. The difference between the requested wrench and this allocated wrench is then passed as an additional feedback channel to the low-level controller, and over time is driven to zero. More details on how this allocated wrench is produced are described in [Szmuk Dissertation, Ch. 6]. The allocator also produces a force vector from each of the actuators, which is then passed into a converter at the lowest software-layer of the high-order controller. This converter models the relationship between the requested set of rotor forces, and the input PWM signal that will produce this set of forces for the physical actuators. Finally, the converter outputs the necessary PWM signals to the rotors, which controls the vehicle along the desired trajectory in the closest dynamically feasible motion to the requested motion. The discrepancy between the translational motion and attitude coupling is negligible when conducting flight experiments.

1. PVA traj, have PID gains that look at the error in position, velocity and feedforward acceleration, and adding all those together we obtain commanded acceleration… May not adhere exactly to interfaces as written there. Magnitude of this accel (force) vector goes into Z channel, normalize vector. Attitude projects that into inertial with normalized vector (attitude controller). Caveats: Attitude in general won’t be exactly as commanded due to time constant. Must make a decision when attitude isn’t as commanded, what should be done about the force. To get aggressive tracking close to the ground, look at what attitude currently is and command acceleration to be what keeps commanded vertical acceleration.
2. Low level controller rejects disturbances and errors of low level. If you don’t follow exactly path that you wanted to, will incur errors at other levels of hierarchy. If attitude is off from plan, then position will drift, so will velocity…. All levels have to play cleanup. High level have to augment the error correction in addition to low level control. Integration of error, CEO, has to be addressed at high level.


==> experiment/figs/diagram.tex <==
\begin{figure}[!ht]
    \centering
    \begin{tikzpicture}
    

 
\node [draw,
    minimum width=1.5cm,
    minimum height=1.2cm
]  (controller) {\scriptsize Controller};


\node[left=0.5cm of controller] (trajectory) {};

\draw[-stealth] (trajectory.east) -- (controller.west) 
    node[at start,left]{\scriptsize trajectory};

\node[draw, minimum width=1.5cm,
    minimum height=1.2cm, right=0.5cm of controller,align=center] (converter)
    {\scriptsize Allocator \\ \scriptsize \&\\ \scriptsize Converter};
    
\draw[-stealth] (controller.east) -- (converter.west);    
 
\node[draw, minimum width=1.5cm,
    minimum height=1.2cm, right=0.5cm of converter] (quadrotor)
    {\includegraphics[width=0.1\textwidth,angle=0,origin=c]{experiment/figs/quad.png}};
    %{\scriptsize Quadrotor};
    
\draw[-stealth] (converter.east) -- (quadrotor.west); 

\node[draw, minimum width=1.5cm,
    minimum height=1.2cm, below=0.5cm of converter] (sensor)
    {\scriptsize Sensors};
 
\draw[-stealth] (quadrotor.south) |- (sensor.east); 

\draw[-stealth] (sensor.west) -| (controller.south);
 
\end{tikzpicture}
    \caption{Feedback control architecture.}
    \label{fig: diagram}
\end{figure}



==> experiment/figs/frame.tex <==
\begin{figure}[!ht]
    \centering
    \begin{tikzpicture}
    \coordinate (A) at (4, 1);
    \coordinate (B) at (0, 0);
    
    
    \node[inner sep=0pt] (sys1) at ($(A)+(0, 0)$)
    {\includegraphics[width=0.15\textwidth,angle=30,origin=c]{feedback/figs/quad.png}};
    
    \draw[-latex, blue] (A) -- ($(A)+(0:1.2)$) node[right] {\footnotesize y-axis};
    \draw[-latex, blue] (A) -- ($(A)+(-120:1.2)$) node[below] {\footnotesize x-axis};
    \draw[-latex, blue] (A) -- ($(A)+(120:1.2)$) node[above] {\footnotesize z-axis};
    
    \draw[-latex] (B) -- ($(B)+(0:1.5)$) node[right] {\footnotesize y-axis};
    \draw[-latex] (B) -- ($(B)+(-120:1)$) node[below] {\footnotesize x-axis};
    \draw[-latex] (B) -- ($(B)+(90:1.5)$) node[above] {\footnotesize z-axis};
    
    \draw[dashed] (A) -- (B);
    
    \fill[blue] (A) circle [radius=1pt]; 
    \fill[black] (B) circle [radius=1pt]; 
    
\end{tikzpicture}
\caption{Intertial frame of reference (black) and body frame of reference (blue).}
\label{fig: body frame}
\end{figure}

==> scribbles.tex <==
To answer the above question, we consider the following \emph{state-transfer problem} for corridor \(\mathbb{H}_i\) (\(i\in[1, l]\)), where (recall the definition of \(\mathbb{H}_i\) in \eqref{eqn: cylinder})
\begin{equation}\label{eqn: p2p boundary}
\begin{aligned}
    &\hat{r}_0\coloneqq c_i-\eta_i d_i,\enskip \hat{r}_f\coloneqq c_i+\eta_i d_i,\enskip \hat{u}_f\coloneqq -mg,\\
    & \hat{v}_0 =\begin{cases}
    \overline{v}_0, & i=1,\\
    \overline{v}_f, & i=l,\\
    0_3, & \text{otherwise}.
    \end{cases}
\end{aligned}    
\end{equation}

An optimal thrust trajectory for optimization~\eqref{opt: pt2pt} steer the quadrotor from its initial state at position \(\hat{r}_0\) to a hovering state at position \(\hat{r}_f\) and stay hovering afterwards. The smallest integer \(\kappa\in\mathbb{N}\) that makes optimization~\eqref{opt: pt2pt} feasible is the minimum value of a quasiconvex function, and one can compute it using a bisection search method that repeatedly test whether optimization~\eqref{opt: pt2pt} is feasible for a given value of \(\kappa\) \cite[Sec. IV-A]{yu2021proportionalB}.  

\vspace{1em}
\noindent\fbox{
\centering
\parbox{0.94\linewidth}{
{\bf{State-transfer problem}}
\begin{equation}\label{opt: pt2pt}
    \begin{array}{ll}
        &\underset{u_{[0, t]}}{\mbox{minimize}} \enskip \frac{1}{2}\sum_{k=0}^t \norm{u_k}^2+\frac{\omega}{2}\sum_{k=0}^{t-1} \norm{u_{k+1}-u_k}^2\\
        &\mbox{subject to} \\ &r_{k+1}=r_k+\Delta v_k+\frac{\Delta^2}{3 m}(u_k+\frac{1}{2}u_{k+1})+\frac{\Delta^2}{2}g,\\
        &v_{k+1}=v_k+\frac{\Delta}{2m}(u_k+u_{k+1})+\Delta g, \enskip \forall k\in[0, t-1],\\
        & u_{k+1}-u_k\in\mathbb{W}, \enskip \forall k\in[0, t-1],\\
       &u_k\in\mathbb{U},\enskip v_k\in\mathbb{V}, \enskip r_k\in \mathbb{H},\enskip \forall k\in[1, \kappa-1],\\
       & r_0=\hat{r}_0, \enskip v_0=\hat{v}_0,\\
       & r_k=\hat{r}_f, \enskip v_k=0_3, \enskip u_k=\hat{u}_f,\enskip  \forall k\in[\kappa, t].
    \end{array}
\end{equation}
}
}
\vspace{1em}

Algorithm~\ref{alg: trigger} computes the triggering time sequence \(\tau_{[0, l]}\) using bisection search method and solving the corresponding instance of optimization~\eqref{opt: trigger}. Its for-loop iterations between line~\ref{alg: trigger start} and line~\ref{alg: trigger end} computes the triggering time sequence \(\tau_{[0, l]}\) recursively. Within this for-loop, the while-loop iterations between line~\ref{alg: bisec start} and line~\ref{alg: bisec end} is a bisection search method for computing the minimum time needed to traverse each corridor; each iteration test whether optimization~\eqref{opt: pt2pt} is feasible given the current value of \(\kappa\). Finally, line~\ref{alg: solve trigger} solves optimization~\eqref{opt: trigger} using the computed triggering time sequence \(\tau_{[0, l]}\) and return the optimal thrust trajectory \(u_{[0, t]}\).  

